Generative Design of Periodic Orbits in the Restricted Three-Body Problem

The Three-Body Problem has fascinated scientists for centuries and it has been crucial in the design of modern space missions. Recent developments in Generative Artificial Intelligence hold transformative promise for addressing this longstanding problem. This work investigates the use of Variational Autoencoder (VAE) and its internal representation to generate periodic orbits. We utilize a comprehensive dataset of periodic orbits in the Circular Restricted Three-Body Problem (CR3BP) to train deep-learning architectures that capture key orbital characteristics, and we set up physical evaluation metrics for the generated trajectories. Through this investigation, we seek to enhance the understanding of how Generative AI can improve space mission planning and astrodynamics research, leading to novel, data-driven approaches in the field.

==> guide.tex <==
\section{Template description (discard)}
\subsection{Subsection}

\subsubsection{My first subsubsection}

Hello there! This is the LaTeX template for the SPAICE conference 2024. In the following, you will find some guidelines as well as typesetting hints (additional information can often be found as comments in the main.tex file).

First a general hint regarding the structure of your paper. \textbf{Every paper has to contain an abstract, an introduction section, a results section and a discussion section.} You can add intermediate and/or subsections as required. \textbf{Please do not change the style of this template}.

Next, some general hints on how to add bibliography, figures, equations, and so on. If you want to cite an article, \textbf{you have to copy its BibTex entry into the 'library.bib' file} included in this folder.
These Bibtex entries can be obtained, e.g., from google scholar.
\textbf{To cite an article, use the cite command}, e.g., \cite{izzo2022selected}. The reference will be added automatically to the reference section.

Figures are added using the figure environment (see source code in main.tex), and can either be single or double column.
% Double column example
% [t] puts the figure at the top of the page, [b] at the  bottom, [h] tries to place it here.
% by setting width between 0 and 1, the size of the image can be changed.
% Text can be added in the \caption{} field.
% Figures have to be put into the figures folder to be accessible here.
\begin{figure*}[t]
    \centering
    \includegraphics[width=.95\textwidth]{figures/image.png}
	\caption{Diagram of the Circular Restricted Three Body Problem}
	\label{fig:voyager_doublecolumn}
\end{figure*}
%
% Single column example (no * behind figure)
\begin{figure}[t]
    \centering
    \includegraphics[width=.95\columnwidth]{figures/voyager.jpg}
	\caption{Example of a single column image.
	}
	\label{fig:voyager_singlecolumn}
\end{figure}
%
Every figure can be given a label, which can be used to \textbf{reference it using the cref command}, e.g., \cref{fig:voyager_singlecolumn,fig:voyager_doublecolumn}.
Please ensure that \textbf{text and labels are large enough} to be readable in the printed version. In addition, please try to not only rely on colours (or use appropriate colours) to \textbf{ensure that people with (partial) colour blindness can read your plots}.
You can add figures in various formats, e.g., pdf, png, and jpeg.

Single line equations are added using the equation environment
%
\begin{equation}
  e^{i \pi} = -1  \,, \label{eq:eidentity}
\end{equation}
%
and can also be assigned a label to be referenced using the cref command, i.e., \cref{eq:eidentity}.

For multi-line equations, use align:
%
\begin{align}
    (a+b)^2 - 2\cdot ab &= a^2 + b^2 + 2 \cdot a b - 2 \cdot a b \,, \\
    &= a^2 + b^2 \,, \\
    &= \frac{1}{2} \cdot 2 \cdot \left(a^2 + b^2 \right) \,. \label{eq:binomial}
\end{align}
%
The lines are aligned using \&. The math syntax of LaTeX is rather similar to the one in Microsoft Word. If you have trouble, try googling commands or ask ChatGPT.

Last but not least, an example of a table.
%
% You can add more columns by adding
% \begin{tabular}{c || c | c | c} more entries here.
% c centers the column content, l and r shifts it left or right.
% | adds a vertical line, || adds a double line.
% Column entries are separated by &.
% Horizontal lines are added using \hline.
\begin{table}[h]\renewcommand{\arraystretch}{1.2}
\begin{center}
\begin{tabular}{c || c | c } 
\hline\hline
Model & RMSE $[10^{-2}]$ & RMSE $[10^{-2}]$\\
\hline\hline
Lin. Regr. & $2.22$ & $15.00$ \\
ANN & $1.00$ & $0.82$ \\
\hline\hline
\end{tabular}
\caption{This is the caption.}
\label{tab:results}
\end{center}
\end{table}
%
By labelling the table, you can cite it again using cref (\cref{tab:results}). Contents of the table should not be in bold or italic face.
\textbf{Please try to adhere to the table style provided here.}

For all references, please \textbf{use the cref command} to ensure a uniform style. Similarly, for citations, \textbf{use the cite command}. 

\textbf{Please do not add page numbers! We will add numbers as well as paper DOIs for the final conference proceedings.}
Additional hints on how to use the syntax can be found as comments in the 'main.tex' file.
